Hierarchical Policy Blending As Optimal Transport

We present hierarchical policy blending as optimal transport (HiPBOT). HiPBOT hierarchically adjusts the weights of low-level reactive expert policies of different agents by adding a look-ahead planning layer on the parameter space. The high-level planner renders policy blending as unbalanced optimal transport consolidating the scaling of the underlying Riemannian motion policies. As a result, HiPBOT effectively decides the priorities between expert policies and agents, ensuring the task's success and guaranteeing safety. Experimental results in several application scenarios, from low-dimensional navigation to high-dimensional whole-body control, show the efficacy and efficiency of HiPBOT. Our method outperforms state-of-the-art baselines -- either adopting probabilistic inference or defining a tree structure of experts -- paving the way for new applications of optimal transport to robot control. More material at https://sites.google.com/view/hipobot

==> acronyms.tex <==
\newacronym{ebm}{EBM}{Energy Based Models}
\newacronym{nce}{NCE}{Noise Contrastive Estimation}

\newacronym{promp}{ProMP}{Probabilistic Movement Primitives}
\newacronym{gp}{GP}{Gaussian Process}
\newacronym{vae}{VAE}{Variational Autoencoder}
\newacronym{gan}{GAN}{Generative Adversarial Network}
\newacronym{chomp}{CHOMP}{Covariant Hamiltonian Optimization for Motion Planning}
\newacronym{stomp}{STOMP}{Stochastic Trajectory Optimization for Motion Planning}
\newacronym{gpmp}{GPMP}{Gaussian Process Motion Planning}
\newacronym{sgpmp}{StochGPMP}{Stochastic Gaussian Process Motion Planning}

\newacronym{map}{MAP}{\textit{maximum a-posteriori}}

\newacronym{cd}{CD}{Contrastive Divergence}

\newacronym{mle}{MLE}{Maximum Likelihood Estimation}
\newacronym{mcmc}{MCMC}{Markov Chain Monte Carlo}

\newacronym{ioc}{IOC}{Inverse Optimal Control}
\newacronym{irl}{IRL}{Inverse Reinforcement Learning}


\newacronym{poe}{PoE}{product of experts}
\newacronym{kld}{KL divergence}{Kullback–Leibler divergence}

\newacronym{rmp}{RMP}{Riemannian motion policies}
\newacronym{rmpflow}{RMP\textit{flow}}{Riemannian motion policies}
\newacronym{mpcicem}{iCEM-MPC}{improved cross entropy method for model-predictive-control}
\newacronym{icem}{iCEM}{improved cross entropy method}
\newacronym{mpc}{MPC}{model predictive control}
\newacronym{hipbi}{HiPBI}{hierarchical policy blending as inference}
